Axions in Cold Dark Matter and Inflation Models

The subjects of this thesis are the invisible axion and the more general family of axion-like particles. The invisible axion is a hypothetical elementary particle and a cold dark matter candidate. I present an improved computation of the constraints on the parameter space of the cold dark matter axion in the standard cosmology, that includes the contributions from anharmonicities in the axion potential and from the decay of axionic strings. In this scenario, I update the value of the mass of the cold dark matter axion, finding the value $(67\pm17){\rm \mu eV}$, approximately one order of magnitude larger than previous computations. The effect of nonstandard cosmological scenarios on the parameter space of axion cold dark matter is studied for the first time. In particular, I consider the cases of low-temperature reheating and kination cosmologies, and I show that the mass of the cold dark matter axion can differ from the value in the standard cosmological scenario by orders of magnitude. Finally, I consider the family of axion-like particles, assuming that these particles serve as the inflaton in the context of warm inflation. I find that the axion energy scale $f$, which in the standard inflation scenario is of the order of the Planck mass, can be lowered to the much safer Grand Unification Theory scale $f \sim 10^{16}{\rm GeV}$. I also constrain the parameter space and the amount of gravitational waves from this model, using results from the Wilkinson Microwave Anisotropy Probe 7-year data.

==> abbreviations.tex <==
\begin{table}{b}
\begin{tabular}{l|l}
BAO & Baryon Acoustic Oscillations\\
BBN & Big Bang nucleosynthesis \\
DM & Dark Matter\\
CDM & Cold Dark Matter\\
CMBR & Cosmic Microwave Background Radiation\\
FRW & Friedmann-Robertson-Walker\\
MSSM & Minimal supersymmetric standard model\\
NFW & Navarro-Frenk-White\\
PNGB & Pseudo Nambu-Goldstone Boson\\
SM & Standard model (of particle physics)\\
SN & Supernova\\
WIMP & Weakly interacting massive particle\\
WMAP & Wilkinson Microwave Anisotropy Probe\\
\end{tabular}
\end{table}


==> abstract.tex <==

The subjects of this thesis are the invisible axion and the more general family of axion-like particles.

The invisible axion is a hypothetical elementary particle and a cold dark matter candidate. I present an improved computation of the constraints on the parameter space of the cold dark matter axion in the standard cosmology, that includes the contributions from anharmonicities in the axion potential and from the decay of axionic strings. In this scenario, I update the value of the mass of the cold dark matter axion, finding the value $(67\pm17){\rm \mu eV}$, approximately one order of magnitude larger than previous computations.

The effect of nonstandard cosmological scenarios on the parameter space of axion cold dark matter is studied for the first time. In particular, I consider the cases of low-temperature reheating and kination cosmologies, and I show that the mass of the cold dark matter axion can differ from the value in the standard cosmological scenario by orders of magnitude.

Finally, I consider the family of axion-like particles, assuming that these particles serve as the inflaton in the context of warm inflation. I find that the axion energy scale $f$, which in the standard inflation scenario is of the order of the Planck mass, can be lowered to the much safer Grand Unification Theory scale $f \sim 10^{16}{\rm GeV}$. I also constrain the parameter space and the amount of gravitational waves from this model, using results from the Wilkinson Microwave Anisotropy Probe 7-year data.

==> acknowledge.tex <==
I would like to thank my advisor, Prof. Paolo Gondolo, for his encouragement and enthusiasm whenever a new project was taking off, and for his support during the developing stages of each work.

I am also indebted to my committee members, Yong-Shi Wu, Wayne Springer, Oleg Starykh, and Aaron Bertram, for their valuable time.

I would like to thank my family - my mother, Giovanna, and my sister, Laura - for their love and support during my odyssey in Utah. They have always encouraged me towards excellence.

Finally, and most importantly, I would like to thank my wife Erika. Her support, patience, encouragement, and unwavering love were undeniably the milestone upon which the past five years of my life have been built.


==> acronyms.tex <==
\begin{acronym}
\acro{ADMX}{Axion dark matter experiment}
\acro{BAO}{Baryon acoustic oscillations}
\acro{BBN}{Big Bang nucleosynthesis}
\acro{CDM}{Cold dark matter}
\acro{CMBR}{Cosmic microwave background radiation}
\acro{COBE}{Cosmic background explorer}
\acro{DFSZ}{Dine-Fischler-Srednicki-Zhitnitsky}
\acro{FRW}{Friedmann-Robertson-Walker}
\acro{GR}{General relativity}
\acro{GUT}{Grand unification theory}
\acro{KSVZ}{Kim-Shifman-Vainshtein-Zakharov}
\acro{LTR}{Low temperature reheating}
\acro{MSSM}{Minimal supersymmetric standard model}
\acro{NWI}{Natural warm inflation}
\acro{QCD}{Quantum chromodynamics}
\acro{QED}{Quantum electrodynamics}
\acro{QFT}{Quantum field theory}
\acro{SN}{Supernova}
\acro{WMAP}{Wilkinson microwave anisotropy probe}
\end{acronym}


==> appA.tex <==

\chapter{Understanding Research Papers}

Appendices follow the same page-numbering rules as regular chapters.
The first page of a multi-page appendix is not numbered. But the page
of a single-page appendix \emph{is} numbered.

A brief introduction to typical phrases used in publications by research
scholars. By Robert Oeffner. http://www.oeffner.net/researchpapers.htm

\begin{longtable}{|>{\raggedright}p{0.5\columnwidth}|>{\raggedright}p{0.5\columnwidth}|}
\hline 
\textbf{They write} & \textbf{They mean}\tabularnewline
\hline
\hline
\endhead
\hline 
\textbf{They write} & \textbf{They mean}\tabularnewline
\hline
\endfirsthead
\hline 
It has long been known that... & I haven't bothered to look up the reference\tabularnewline
\hline 
...of great theoretical and practical importance & ...interesting to me\tabularnewline
\hline 
While it has not been possible to provide definite answers to these
questions... & The experiments didn't work out, but I figured I could at least get
a publication out of it...\tabularnewline
\hline 
The W-Pb system was chosen as especially suitable to show the predicted
behavior... & The fellow in the next lab had some already made up\tabularnewline
\hline 
High purity...

Very high purity...

Extremely high purity...

Super-purity...

Spectroscopically pure... & Composition unknown except for exaggerated claims of the supplier\tabularnewline
\hline 
A fiducial reference line... & A scratch\tabularnewline
\hline 
Three of the samples were chosen for detailed study... & The results of the others didn't make sense and were ignored...\tabularnewline
\hline 
...handled with extreme care during the experiments & ...not dropped on the floor\tabularnewline
\hline 
Typical results are shown... & The best results are shown...\tabularnewline
\hline 
Although some detail has been lost in reproduction, it is clear from
the original micrograph & It is impossible to tell from the micrograph\tabularnewline
\hline 
Presumably at longer times... & I didn't take the time to find out\tabularnewline
\hline 
The agreement with the predicted curve is:

excellent

good

satisfactory

fair

...as good as could be expected & ~

fair

poor

doubtful

imaginary

non-existent\tabularnewline
\hline 
These results will be reported at a later date & I might get around to this sometime\tabularnewline
\hline 
The most reliable values are those of Jones & Jones was a student of mine\tabularnewline
\hline 
It is suggested that...

It is believed taht...

It may be that... & I think...\tabularnewline
\hline 
It is generally believed that... & I have such a good objection to this answer that I shall now raise
it\tabularnewline
\hline 
It is clear that much additional work will be required before a complete
understanding... & I don't understand it\tabularnewline
\hline 
Unfortunately, a quantitative theory to account for these effects
has not been formulated & Neither does anybody else\tabularnewline
\hline 
Correct within an order of magnitude & Wrong\tabularnewline
\hline 
It is hoped that this work will stimulate further work in the field & This paper isn't very good but neither are any of the others on this
miserable subject\tabularnewline
\hline 
Thanks are due to Joe Glotz for assistance with the experiments and
to John Doe for valuable discussions & Glotz did the work and Doe explained what it meant\tabularnewline
\hline
\end{longtable}




==> appB.tex <==

\chapter{Another Appendix Example}

 


==> notation.tex <==

\begin{table}[b!]
\hbox{We use natural units $\hbar = c = \epsilon_0 = \mu_0 = k_B = 1$}
\hbox{}
\begin{tabular}{llll|}
$\alpha$ & Spinor index; Fine structure constant; Parameter used in chapter~\ref{Natural warm inflation}, see Eq.~(\ref{def_alpha}).\\
$\alpha_s$ & Structure constant for the strong interactions.\\
$\alpha_{af}$ & Structure constant for Yukawa interactions.\\
$\alpha_0$ & Axion adiabaticity.\\
$\beta$ & Spinor index; Dirac matrix in Eq.~(\ref{beta_matrix}); Parameter in non-standard cosmologies, Eq.~(\ref{a(t)}).\\
$\beta_H$ & Ratio of two Higgs vacuum expectation values in the DFSZ model.\\
$\gamma$ & Label for the photon; Parameter in Eq.~(\ref{anharmonicities}); function in Eq.~(\ref{yamaguchi}).\\
$\gamma^\mu$ & Dirac matrices.\\
$\gamma^5$ & Product of the four Dirac matrices, $\gamma^5 = i\gamma^0\gamma^1\gamma^2\gamma^3$.\\
$\delta$ & Axionic string core size.\\
$\delta_\mu^\nu$ & Identity matrix.\\
$\epsilon$ & First slow-roll parameter.\\
$\epsilon_{ijk}$ & Completely antisymmetric tensor in three dimensions.\\
$\epsilon_{\mu\nu\sigma\rho}$ & Completely antisymmetric tensor in four dimensions.\\
$\zeta$ & Uncertainties in the spectrum of axions radiated from strings.\\
$\eta$ & Second slow-roll parameter.\\
$\eta_{\mu\nu}$ & Metric in flat space-time.\\
$\theta$ & Elevation angle on a sphere; Axion misalignment angle.\\
$\lambda_\phi$ & Quartic self-interaction of the inflaton field.\\
$\mu$ & Four-vector index.\\
$\nu$ & Four-vector index; Parameter in the $T$-dependent axion mass, see Eq.~(\ref{bae_mass}).\\
$\xi$ & Bi-spinor.\\
$\rho$ & Four-vector index; Energy density.\\
$\rho_c$ & Critical density of the universe at the present time.\\
$\rho_i$ & Energy density of the $i$-th fluid.\\
$\sigma$ & Four-vector index.\\
$\sigma^i$ & Pauli matrices.\\
$\tau$ & Conformal time.\\
$\phi(x)$ & Inflaton field.\\
$\chi$ & Bi-spinor; Fudge factor in the axion number density, Eq.~(\ref{number_density})\\
$\omega$ & Parameter of U(1) transformation, Eq.~(\ref{U1_transformation});  Parameter in Eq.~(\ref{anharmonicities}).\\
$\omega(t)$ & Average energy of axions radiated in the decay of strings at time $t$.
\end{tabular}
\end{table}

\begin{table}[tb]
\begin{tabular}{llll|}
$\Gamma$ & Dissipative term in the warm inflation scenario.\\
$\Gamma^\sigma_{\mu\nu}$ & Levi-Civita connection.\\
$\Delta^2_{\mathcal{R}}(k)$ & Power spectrum for density perturbations at wavelength $k$.\\
$\Delta^2_{\mathcal{T}}(k)$ & Power spectrum for tensor perturbations at wavelength $k$.\\
$\Lambda$ & Cosmological constant; Energy scale in axion-like theories.\\
${\Lambda^\mu}_\nu$ & Representation of the Lorentz transformation.\\
$\Lambda_{\rm QCD}$ & QCD energy scale.\\
$\Phi(x)$ & Generic scalar field.\\
$\Psi(x)$ & Generic spinor field.\\
$\Omega_i$ & Energy density of the $i$-th species in units of the critical density $\rho_c$.\\
$\Omega_{\rm tot}$ & Total energy density in units of the critical density $\rho_c$.\\
$a$ & Index of a Lie group.\\
$a(x)$ & Axion field.\\
$a(t)$ & Scale factor at time $t$.\\
$a_0$ & Scale factor at the present time.\\
$f$ & Decay constant in axion-like theories.\\
$f_a$ & Decay constant in invisible axion theories.\\
$g_{\mu\nu}$ & Generic metric in curved space-time.\\
$g_{a\gamma}$ & Axion-photon coupling.\\
$i,j,k$ & Spatial coordinates.\\
$m_a$ & Mass of the invisible axion at zero temperature.\\
$m_a(T)$ & Mass of the invisible axion at temperature $T$.\\
$n_s$ & Scalar spectral index.\\
$n_T$ & Tensor spectral index.\\
$p_i$ & Pressure of the $i$-th fluid.\\
$q_n$ & Quark field with flavor $n$.\\
$r$ & Tensor-to-scalar ratio.\\
$t_0$ & Age of the universe.\\
$v^i$ & $i$-th component of a three-vector $v$.\\ 
$w_i$ & Parameter specifying the equation of state for the $i$-th fluid.\\
$x^\mu$ & $\mu$-th component of a four-vector $x$.\\
$z$ & Redshift.\\
$G^{\mu\nu a}$ & Gluon field.\\
$H, H(t), H(T)$ & Hubble expansion rate at time $t$ or at temperature $T$.\\
$H_I$ & Hubble expansion rate at the end of inflation.\\ 
$H_0$ & Hubble expansion rate at the present time.\\ 
$J_i$ & Generator of the angular momentum.\\
$K_i$ & Generator of the boost symmetry.\\
$M$ & Quark mass matrix.\\
$M_{\rm Pl}$ & Planck mass.\\
$N$ & Peccei-Quinn color anomaly.\\
$N_e$ & Number of e-folds.\\
$N_f$ & Number of relativistic quarks at temperature $T$.\\
$T^a$ & Generator of a Lie group.\\
$T_0$ & CMBR temperature at the present time.\\
$U$, $V(\phi)$ & Axion potential in axion-like theories.\\
$V$, $V(\theta)$ & Axion potential in invisible axion theories.\\
\end{tabular}
\end{table}
\acro{$\alpha$}{Spinor index; Fine structure constant; Parameter used in chapter~\ref{Natural warm inflation}, see Eq.~(\ref{def_alpha}).}
\acro{$\alpha_s$}{Structure constant for the strong interactions.}
\acro{$\alpha_{af}$}{Structure constant for Yukawa interactions.}
\acro{$\alpha_0$}{Axion adiabaticity.}
\acro{$\beta$}{Spinor index; Dirac matrix in Eq.~(\ref{beta_matrix}); Parameter in non-standard cosmologies, Eq.~(\ref{a(t)}).}
\acro{$\beta_H$}{Ratio of two Higgs vacuum expectation values in the DFSZ model.}
\acro{$\gamma$}{Label for the photon; Parameter in Eq.~(\ref{anharmonicities}); function in Eq.~(\ref{yamaguchi}).}
\acro{$\gamma^\mu$}{Dirac matrices.}
\acro{$\gamma^5$}{Product of the four Dirac matrices, $\gamma^5 = i\gamma^0\gamma^1\gamma^2\gamma^3$.}
\acro{$\delta$}{Axionic string core size.}
\acro{$\delta_\mu^\nu$}{Identity matrix.}
\acro{$\epsilon$}{First slow-roll parameter.}
\acro{$\epsilon_{ijk}$}{Completely antisymmetric tensor in three dimensions.}
\acro{$\epsilon_{\mu\nu\sigma\rho}$}{Completely antisymmetric tensor in four dimensions.}
\acro{$\zeta$}{Uncertainties in the spectrum of axions radiated from strings.}
\acro{$\eta$}{Second slow-roll parameter.}
\acro{$\eta_{\mu\nu}$}{Metric in flat space-time.}
\acro{$\theta$}{Elevation angle on a sphere; Axion misalignment angle.}
\acro{$\lambda_\phi$}{Quartic self-interaction of the inflaton field.}
\acro{$\mu$}{Four-vector index.}
\acro{$\nu$}{Four-vector index; Parameter in the $T$-dependent axion mass, see Eq.~(\ref{bae_mass}).}
\acro{$\xi$}{Bi-spinor.}
\acro{$\rho$}{Four-vector index; Energy density.}
\acro{$\rho_c$}{Critical density of the universe at the present time.}
\acro{$\rho_i$}{Energy density of the $i$-th fluid.}
\acro{$\sigma$}{Four-vector index.}
\acro{$\sigma^i$}{Pauli matrices.}
\acro{$\tau$}{Conformal time.}
\acro{$\phi(x)$}{Inflaton field.}
\acro{$\chi$}{Bi-spinor; Fudge factor in the axion number density, Eq.~(\ref{number_density})}
\acro{$\omega$}{Parameter of U(1) transformation, Eq.~(\ref{U1_transformation});  Parameter in Eq.~(\ref{anharmonicities}).}
\acro{$\omega(t)$}{Average energy of axions radiated in the decay of strings at time $t$.
\acro{$\Gamma$}{Dissipative term in the warm inflation scenario.}
\acro{$\Gamma^\sigma_{\mu\nu}$}{Levi-Civita connection.}
\acro{\acro{$\Delta^2_{\mathcal{R}}(k)$}{Power spectrum for density perturbations at wavelength $k$.}
\acro{$\Delta^2_{\mathcal{T}}(k)$}{Power spectrum for tensor perturbations at wavelength $k$.}
\acro{$\Lambda$}{Cosmological constant; Energy scale in axion-like theories.}
\acro{${\Lambda^\mu}_\nu$}{Representation of the Lorentz transformation.}
\acro{$\Lambda_{\rm QCD}$}{QCD energy scale.}
\acro{$\Phi(x)$}{Generic scalar field.}
\acro{$\Psi(x)$}{Generic spinor field.}
\acro{$\Omega_i$}{Energy density of the $i$-th species in units of the critical density $\rho_c$.}
\acro{$\Omega_{\rm tot}$}{Total energy density in units of the critical density $\rho_c$.}
\acro{$a$}{Index of a Lie group.}
\acro{$a(x)$}{Axion field.}
\acro{$a(t)$}{Scale factor at time $t$.}
\acro{$a_0$}{Scale factor at the present time.}
\acro{$f$}{Decay constant in axion-like theories.}
\acro{$f_a$}{Decay constant in invisible axion theories.}
\acro{$g_{\mu\nu}$}{Generic metric in curved space-time.}
\acro{$g_{a\gamma}$}{Axion-photon coupling.}
\acro{$i,j,k$}{Spatial coordinates.}
\acro{$m_a$}{Mass of the invisible axion at zero temperature.}
\acro{$m_a(T)$}{Mass of the invisible axion at temperature $T$.}
\acro{$n_s$}{Scalar spectral index.}
\acro{$n_T$}{Tensor spectral index.}
\acro{$p_i$}{Pressure of the $i$-th fluid.}
\acro{$q_n$}{Quark field with flavor $n$.}
\acro{$r$}{Tensor-to-scalar ratio.}
\acro{$t_0$}{Age of the universe.}
\acro{$v^i$}{$i$-th component of a three-vector $v$.} 
\acro{$w_i$}{Parameter specifying the equation of state for the $i$-th fluid.}
\acro{$x^\mu$}{$\mu$-th component of a four-vector $x$.}
\acro{$z$}{Redshift.}
\acro{$G^{\mu\nu a}$}{Gluon field.}
\acro{$H, H(t), H(T)$}{Hubble expansion rate at time $t$ or at temperature $T$.}
\acro{$H_I$}{Hubble expansion rate at the end of inflation.} 
\acro{$H_0$}{Hubble expansion rate at the present time.} 
\acro{$J_i$}{Generator of the angular momentum.}
\acro{$K_i$}{Generator of the boost symmetry.}
\acro{$M$}{Quark mass matrix.}
\acro{$M_{\rm Pl}$}{Planck mass.}
\acro{$N$}{Peccei-Quinn color anomaly.}
\acro{$N_e$}{Number of e-folds.}
\acro{$N_f$}{Number of relativistic quarks at temperature $T$.}
\acro{$T^a$}{Generator of a Lie group.}
\acro{$T_0$}{CMBR temperature at the present time.}
\acro{$U$, $V(\phi)$}{Axion potential in axion-like theories.}
\acro{$V$, $V(\theta)$}{Axion potential in invisible axion theories.}

